ReFit: Recurrent Fitting Network for 3D Human Recovery

We present Recurrent Fitting (ReFit), a neural network architecture for single-image, parametric 3D human reconstruction. ReFit learns a feedback-update loop that mirrors the strategy of solving an inverse problem through optimization. At each iterative step, it reprojects keypoints from the human model to feature maps to query feedback, and uses a recurrent-based updater to adjust the model to fit the image better. Because ReFit encodes strong knowledge of the inverse problem, it is faster to train than previous regression models. At the same time, ReFit improves state-of-the-art performance on standard benchmarks. Moreover, ReFit applies to other optimization settings, such as multi-view fitting and single-view shape fitting. Project website: https://yufu-wang.github.io/refit_humans/

==> figs/fig_results.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.12\textwidth]{figs/results/image14.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image21.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image28.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image30.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image36.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image33.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image59.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image57.png}\\
    \includegraphics[width=0.12\textwidth]{figs/results/image12.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image19.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image26.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image24.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image40.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image38.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image77.png}
    \includegraphics[width=0.12\textwidth]{figs/results/image74.png}\\
    \vspace{-2mm}
    \caption{{\bf Qualitative comparison of regression-based methods.}}
    \label{fig:results}
    \vspace{-2mm}
\end{figure*}

==> figs/fig_results2.tex <==
\begin{figure*}[!t]
\vspace{-1mm}
\captionsetup[subfigure]{labelformat=empty}
    \centering
    \begin{subfigure}[t]{0.245\textwidth}
    \caption{ \textbf{30$^{\text{th}}$ percentile }}
            \includegraphics[width=0.49\textwidth]{figs/results/image14.png}
            \includegraphics[width=0.49\textwidth]{figs/results/image21.png}
   \end{subfigure}
    \begin{subfigure}[t]{0.245\textwidth}
    \caption{ \textbf{60$^{\text{th}}$ percentile }}
            \includegraphics[width=0.49\textwidth]{figs/results/image28.png}
            \includegraphics[width=0.49\textwidth]{figs/results/image30.png}
   \end{subfigure}
    \begin{subfigure}[t]{0.245\textwidth}
    \caption{ \textbf{90$^{\text{th}}$ percentile }}
            \includegraphics[width=0.49\textwidth]{figs/results/image36.png}
            \includegraphics[width=0.49\textwidth]{figs/results/image33.png}
   \end{subfigure}
    \begin{subfigure}[t]{0.245\textwidth}
    \caption{ \textbf{99$^{\text{th}}$ percentile}}
            \includegraphics[width=0.49\textwidth]{figs/results/image59.png}
            \includegraphics[width=0.49\textwidth]{figs/results/image57.png}
   \end{subfigure}
   \\
    \begin{subfigure}[t]{0.245\textwidth}
            \includegraphics[width=0.49\textwidth]{figs/results/image12.png}
            \includegraphics[width=0.49\textwidth]{figs/results/image19.png}
           \vspace{-6mm}
   \end{subfigure}
    \begin{subfigure}[t]{0.245\textwidth}
            \includegraphics[width=0.49\textwidth]{figs/results/image26.png}
            \includegraphics[width=0.49\textwidth]{figs/results/image24.png}
            \vspace{-6mm}
   \end{subfigure}
    \begin{subfigure}[t]{0.245\textwidth}
            \includegraphics[width=0.49\textwidth]{figs/results/image40.png}
            \includegraphics[width=0.49\textwidth]{figs/results/image38.png}
            \vspace{-6mm}
     \end{subfigure}
    \begin{subfigure}[t]{0.245\textwidth}
            \includegraphics[width=0.49\textwidth]{figs/results/image77.png}
            \includegraphics[width=0.49\textwidth]{figs/results/image74.png}
            \vspace{-6mm}
   \end{subfigure}\\
    \vspace{-2mm}
    \caption{{\bf Qualitative results from ReFit} on 3DPW. Examples are organized by MPJPE percentile. Higher percentile indicates higher error. For example, samples at the 99$^{\text{th}}$ percentile have higher error than 99\% of the examples. The MPJPE at the four percentiles are 50.5mm, 65.4mm, 99.3mm and 158.8mm respectively. Samples at the 99$^{\text{th}}$ percentile often have severe occlusions or cropping.}
    \label{fig:results}
    \vspace{-2mm}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

